Molecular laser cooling using serrodynes: Implementation, characterization and prospects

An important effort is currently underway to extend optical cycling and laser cooling to more molecular species. Significant challenges arise in particular when multiple nuclear spins give rise to complex, resolved hyperfine spectra, as is the case for several molecular species relevant to precision tests of fundamental symmetries. We provide a detailed introduction to the use of optical spectra generated via serrodyne waveforms to address this complexity. We discuss our experimental implementation of these serrodynes, characterize their properties, and outline procedures to find optimized sideband configurations that generate strong laser cooling forces. We demonstrate the application of these techniques to barium monofluoride molecules and explore their prospects for the cooling of other species relevant to the study of fundamental physics.

==> preamble.tex <==
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{physics}
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage[left=23mm,right=13mm,top=35mm,columnsep=15pt]{geometry} 
\usepackage{adjustbox}
\usepackage{placeins}
\usepackage[T1]{fontenc}
\usepackage{lipsum}
\usepackage{csquotes}
